Relational Programming with Foundation Models

Foundation models have vast potential to enable diverse AI applications. The powerful yet incomplete nature of these models has spurred a wide range of mechanisms to augment them with capabilities such as in-context learning, information retrieval, and code interpreting. We propose Vieira, a declarative framework that unifies these mechanisms in a general solution for programming with foundation models. Vieira follows a probabilistic relational paradigm and treats foundation models as stateless functions with relational inputs and outputs. It supports neuro-symbolic applications by enabling the seamless combination of such models with logic programs, as well as complex, multi-modal applications by streamlining the composition of diverse sub-models. We implement Vieira by extending the Scallop compiler with a foreign interface that supports foundation models as plugins. We implement plugins for 12 foundation models including GPT, CLIP, and SAM. We evaluate Vieira on 9 challenging tasks that span language, vision, and structured and vector databases. Our evaluation shows that programs in Vieira are concise, can incorporate modern foundation models, and have comparable or better accuracy than competitive baselines.

==> figures/motivating-example-a-backup.tex <==
\begin{figure}
  \begin{lstlisting}[language=scallop,basicstyle=\sclsizesmall\ttfamily,frame=single,xleftmargin=0.2cm,xrightmargin=0.2cm,framesep=5px,framexleftmargin=0pt,framexrightmargin=0pt]
@gpt("The height of {{x}} is {{y}} in meters")
type height(bound x: String, y: i32)

rel mountain = {"Mt. Everest", "Fuji"}
rel mountain_height(m, h) = mountain(m), height(m, h)
// {("Mt. Everest", 8848), ("Fuji", 3776)}
  \end{lstlisting}
  \vspace{-10px}
  \caption{Using GPT to extract common sense knowledge about height of mountains.}
  \label{fig:moti-a}
  \vspace{-15px}
\end{figure}

% \begin{figure}
%   \begin{subfigure}[b]{\linewidth}
%     \centering
%     % \includegraphics[width=0.85\linewidth]{figures/moti-a.pdf}
%     \begin{lstlisting}[language=scallop,basicstyle=\sclsizesmall\ttfamily,frame=single,framesep=5px,framexleftmargin=0pt,framexrightmargin=0pt]
% @gpt("The height of {{x}} is {{y}} in meters")
% type height(bound x: String, y: i32)

% rel answer(m, h) = mountain(m) and height(m, h)
%     \end{lstlisting}
%     \caption{Extracting common sense knowledge using ChatGPT}
%   \end{subfigure}
%   \begin{subfigure}[b]{\linewidth}
%     \vspace{5px}
%     \centering
%     % \includegraphics[width=0.85\linewidth]{figures/moti-b.pdf}
%     \begin{lstlisting}[language=scallop,basicstyle=\sclsizesmall\ttfamily,frame=single,framesep=5px,framexleftmargin=0pt,framexrightmargin=0pt]
% @clip(["cat", "dog"])
% type classify(bound img: Tensor, label: String)

% rel cat_or_dog(i, l) = image(i, m) and classify(m, l)
%     \end{lstlisting}
%     \caption{Classifying images using CLIP}
%   \end{subfigure}
%   \caption{Programming foundation models under zero-shot settings.}
%   \label{fig:programming-foundation-models}
% \end{figure}


==> figures/motivating-example-b-backup.tex <==
\begin{figure}
  \centering
  \footnotesize
  \begin{subfigure}[c]{0.18\linewidth}
    \centering
    \includegraphics[height=0.9in]{figures/moti-b1.pdf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.42\linewidth}
    \centering
    \begin{lstlisting}[language=scallop,basicstyle=\sclsizetiny\ttfamily,frame=single,xleftmargin=-0.06cm,xrightmargin=0cm,aboveskip=4px]
@clip(["cat", "dog"])
type classify_animal(
  bound img: Tensor,
  free label: String)

// Classify the animals
rel cat_or_dog(i, l) =
  animal_photo(i, m) and
  classify_animal(m, l)
    \end{lstlisting}
  \end{subfigure}
  \hfill
  \begin{subfigure}[c]{0.298\linewidth}
    \centering
    \includegraphics[height=0.9in]{figures/moti-b2.pdf}
  \end{subfigure}
  \vspace{-10px}
  \caption{
    Given the relation \inlinescl{animal\_photo} on the left,
    the \tool{} program in the middle invokes CLIP to classify each image,
    producing the \inlinescl{cat\_or\_dog} relation on the right, in which each fact is associated with a probability.
  }
  \label{fig:moti-b}
  \vspace{-15px}
\end{figure}


==> rebuttal.tex <==
We thank the reviewers for their insightful comments and feedback. We appreciate the consensus among reviewers that the language and idea of Vieira is novel and interesting, and that the paper is well-written. We hereby respond to the reviewers’ questions. Before each question, we specify the reviewers who raised the question.

\paragraph{(R3, R4, R5) Reproducibility, Artifact, and GQA Results}

We provide an anonymized Github repo (vieira-artifact/vieira-artifact-aaai24) containing runnable Jupyter notebooks for all of our presented benchmark tasks. Reviewers can open the notebooks and execute them on platforms like Google Colab. While some tasks require using OpenAI services and thus need an OpenAI API Key, the notebooks still contain the sample output which could be examined without running anything. In addition, the repo contains all the produced logs if the task invokes a language model for textual response. The software of Vieira will be fully open-sourced upon publication.

We thank reviewer \#4 for pointing out the issue with GQA experiments. Upon further investigation, we find that the original number was obtained by evaluating our method on only a limited subset of the samples. After updating the evaluation, we now have results of 0.579 for Recall@1 and 0.665 for Recall@3, compared to 0.79 and 0.89 as stated in our paper. We note that this new result is still better than the mentioned SOTA (0.419) under no-training setting [PNP-VQA, Tiong et. al, 2022]. We will update the camera-ready version with this new result. The reviewers can checkout the provided notebooks \inlinecode{gqa\_full.ipynb} and \inlinecode{gqa\_main.ipynb} in our artifact. In particular, \inlinecode{gqa\_main.ipynb} performs evaluation with our pre-generated GPT-4 outcome, so that results can be reproduced without an OpenAI API key.

\paragraph{(R3) Is there a provision in Vieira to fine-tune the foundation models?}

Yes. As proposed in the conclusion, we are developing an end-to-end fine-tuning framework using techniques from the neuro-symbolic learning community. Currently, not only foundation models but also regular models can be trained under our differentiable framework. The goal is to have Vieira become the de-facto framework for programming, composing, debugging, and fine-tuning foundation models in an end-to-end fashion.

\paragraph{(R3) On the significance of employed DSL}

The DSL plays an important role in the reasoning process, and defines the space of which the LLM and other foundation models can operate on. In our experience, the designing of a DSL containing $<10$ modules is usually straightforward, but it is indeed challenging for a new user. We agree that an experiment on how well new users can design a new DSL is interesting, but would be out-of-scope for this paper. We will add the discussion to the limitations and conclusion section.

\paragraph{(R3) Discussion of the STAR Framework [Rajasekharan et. al, ICLP 2023]}

We thank the reviewer for the suggestion, and we will cite the work in our camera-ready version. Upon reading the paper, we find that there are indeed certain similarities between our work and theirs. But compared to STAR, Vieira incorporates more diverse foundation models (besides LLMs) through an extensible plugin framework, and supports differentiable and probabilistic reasoning.

\paragraph{(R3) In Table 2, is DSL length accounted for?} Yes.

\paragraph{(R3) How many test samples were evaluated for each of the 3, 5, 7 objects?} 

As stated in Appendix C.2, \textasciitilde 20\% of the samples are for $n=3$, and \textasciitilde 40\% are for $n=5$ and $n=7$ each. So the result is indeed statistically significant.

\paragraph{(R4) What would happen when a model does not return a result or when the results do not match the required datatype?} 

For evaluations presented in the paper, we simply discard the result and count the sample as failed. Although not emphasized in the paper, the LLM plugins in Vieira provide additional options for retrying with chain-of-thought prompts and self-reflection prompts, which can help increase the likelihood of success.

\paragraph{(R4) Why was the recall@k metric for the VQA tasks used?} 

Recall@k is the accuracy commonly seen in evaluations of VQA tasks [Kim, Son, and Kim, 2021]. Recall@1 is simply the accuracy.

\paragraph{(R4) What is the exact meaning of ``shots’' in the context of this paper?} It is the number of examples provided to GPT only. Each shot is not an end-to-end input/output pair, but only the expected relational input/output for the language model. In the final version of the paper, we will clarify in the experimental result section.

\paragraph{(R5) Comparing to TaskMatrix.AI or AutoGPT}

We will cite the work and provide a discussion in the related works section. In these approaches, a black-box LLM controls symbolic reasoning, by calling APIs in the case of taskmatrix.ai and by self-correcting in the case of AutoGPT. The programmer can indirectly influence the reasoning process by prompting or fine-tuning the LLM. On the other hand, in Vieira, the programmer directly specifies symbolic reasoning. The former is open-domain but monolithic and hard to control, whereas the latter is modular and deterministic but more domain-specific.

\paragraph{(R5) Importance of relational language}

We thank the reviewer for the suggestion, and we will include the following discussion in the introduction section: Declarative relational languages operate on sets and tuples, and decouple high-level specifications from low-level implementation details. They lift the users from manipulating low-level data-structures, like lists and dictionaries, into a logically intuitive interface of rules and constraints. Hence, we view relational programming as an alternative paradigm that elicits more interpretable neuro-symbolic programs from users.

\paragraph{(R6) How can Vieira adapt to the evolving landscape of AI? How could we seamlessly incorporate Vieira for new models?}

As can be seen from our provided artifact (Q1), the foundation models are provided through Vieira’s plugin system. In particular, models like GPT and Clip are provided through separated plugins. We envision creating a plugin marketplace for Vieira, so that people can create and share new plugins to provide support to the newly created models.

